QCD resummation for high-p$_T$ jet shapes at hadron colliders

Exploiting the substructure of jets observed at the LHC to better understand and interpret the experimental data has recently been a very active area of research. In this thesis we study the substructure of high-p$_T$ QCD jets, which form a background to many new physics searches. In particular, we explore in detail the perturbative distributions of a certain class of observables known as non-global jet shapes. More specifically, we identify and present state-of-the-art calculations, both at fixed-order and to all-orders in the perturbative expansion, of a set of large logarithms known as non-global logarithms. Hitherto, these logarithms have been largely mistreated, and in many cases ignored, in the literature despite being first pointed out more than a decade ago. Our work has triggered the interest of many groups, particularly Soft and Collinear Effective Theory (SCET) groups, and led to a flurry of papers on non-global logarithms and related issues.

==> ch4/ch4app.tex <==
% Chapter 4 Appendix

\chapter{}
